Scale Adaptive Clustering of Multiple Structures

We propose the segmentation of noisy datasets into Multiple Inlier Structures with a new Robust Estimator (MISRE). The scale of each individual structure is estimated adaptively from the input data and refined by mean shift, without tuning any parameter in the process, or manually specifying thresholds for different estimation problems. Once all the data points were classified into separate structures, these structures are sorted by their densities with the strongest inlier structures coming out first. Several 2D and 3D synthetic and real examples are presented to illustrate the efficiency, robustness and the limitations of the MISRE algorithm.

==> alldefin.tex <==
%%%%%%%%  page layout

%\textheight = 8in
%\textwidth = 4.7in
%\evensidemargin= 0.0in
%\oddsidemargin= 0.0in
%\topmargin = - 0.5in
%\headsep = 0.5in
%\columnsep = 0.2in
%\headheight = 0.0in
%\parskip = .1in
%\parindent = 0.4in
\RequirePackage{xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother



\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbQ}{\mathbb{Q}}

\newcommand{\GL}[1]{\mbox{$\mathbf{GL}(#1)$}}
\newcommand{\SL}[1]{\mbox{$\mathbf{SL}(#1)$}}
\newcommand{\SE}[1]{\mbox{$\mathbf{SE}(#1)$}}
\newcommand{\se}[1]{\mbox{\tengoth{se}(#1)}}
\newcommand{\SO}[1]{\mbox{$\mathbf{SO}(#1)$}}
\newcommand{\so}[1]{\mbox{\tengoth{so}(#1)}}
\newcommand{\Af}[1]{\mbox{$\mathbf{A}(#1)$}}
\newcommand{\Grass}[2]{\mathbf{G}_{#1,#2}}
\newcommand{\Sym}[1]{Sym_{#1}^{+}}

\newcommand{\X}{\mbox{$\bf X$}}

\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Tan}[2]{T_{#1}(#2)}
\newcommand{\func}[1]{\mathfrak{F}(#1)}
\newcommand{\vecf}[1]{\mathfrak{X}(#1)}



\newcommand{\SSS}{\scriptscriptstyle}
\newcommand{\vc}[1]{\mbox{\boldmath ${#1}$}}

%%%%%%%%%%%mine%%%%%%%%%%%%%%%%%%%%
\newcommand{\eye}[1]{\mbox{\boldmath $\bf{e}_{#1}$}}
\newcommand{\zio}{\vc{z}_{io}}
\newcommand{\zi}{\vc{z}_{i}}
\newcommand{\zihat}{\hat{\vc{z}}_{i}}
\newcommand{\zicheck}{\check{\vc{z}}_{i}}
\newcommand{\zj}{\vc{z}_{j}}
\newcommand{\zjhat}{\hat{\vc{z}}_{j}}
\newcommand{\zjcheck}{\check{\vc{z}}_{j}}
\newcommand{\ro}{\vc{r}_{o}}
\newcommand{\rr}{\vc{r}}
\newcommand{\rhat}{\hat{\vc{r}}}
\newcommand{\rcheck}{\check{\vc{r}}}
\newcommand{\tv}{\vc{t}}
\newcommand{\that}{\hat{\vc{t}}}
\newcommand{\Covmat}{\vc{C}}
\newcommand{\bvarphi}{\mbox{\boldmath $\varphi$}}
\newcommand{\mydef}{\stackrel{\Delta}{=}}
\newcommand{\f}{\mbox{$\vc f$}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ftilde}{\tilde{f}}

%\renewcommand{\labelitemi}{} %{--}
\newfont{\tengoth}{eufm10}
\newcommand{\lieg}{\mbox{\tengoth{g}}}
\newcommand{\lieh}{\mbox{\tengoth{h}}}

\newcommand{\luv}{$\rm \  L^{*}u^{*}v^{*} \  $}
\newcommand{\lab}{$\rm \  L^{*}a^{*}b^{*} \  $}

\newcommand{\trans}{^{\top}}

\newcommand{\myrfe}[1]{(\ref{eqn:#1})}
\newcommand{\myrff}[1]{\ref{fig:#1}}
\newcommand{\myrfs}[1]{\ref{sec:#1}}
\newcommand{\myrft}[1]{\ref{tab:#1}}

\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bLambda}{\mbox{\boldmath $\Lambda$}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\balphahat}{\mbox{\boldmath $\hat{\alpha}$}}
\newcommand{\alphahat}{\mbox{$\hat{\alpha}$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bSigmahat}{\mbox{\boldmath $\hat{\Sigma}$}}
\newcommand{\boldeta}{\mbox{\boldmath $\eta$}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bthetahat}{\mbox{\boldmath $\hat{\theta}$}}
\newcommand{\bthetacheck}{\mbox{\boldmath $\check{\theta}$}}
\newcommand{\bthetahathat}{\mbox{\boldmath $\hat{\hat{\theta}}$}}
\newcommand{\bthetabar}{\mbox{\boldmath $\bar{\theta}$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\bThetahat}{\mbox{\boldmath $\hat{\Theta}$}}
\newcommand{\bldomega}{\mbox{\boldmath $\omega$}}
\newcommand{\boldpi}{\mbox{\boldmath $\pi$}}
\newcommand{\bbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bbetahat}{\mbox{\boldmath $\hat{\beta}$}}
\newcommand{\bPsi}{\mbox{\boldmath $\Psi$}}
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bnu}{\mbox{\boldmath $\nu$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\talpha}{\tilde\alpha}
\newcommand{\tgamma}{\tilde\gamma}
\newcommand{\teta}{\tilde\eta}

\newcommand{\bomega}{\mbox{\boldmath $\omega$}}
\newcommand{\vomega}{\vc{\omega}}

\newcommand{\vyhat}{\hat{\vc{y}}}
\newcommand{\x}{\vc{x}}
\newcommand{\y}{\vc{y}}
\newcommand{\ty}{\tilde\y}
\newcommand{\tbC}{\tilde{\bf C}}

\newcommand{\tbx}{\tilde{\vc{x}}}
\newcommand{\tbX}{\tilde{\vc{X}}}
\newcommand{\bl}{\mbox{$\mathbf{l}$}}
\newcommand{\tbe}{\tilde{\vc{e}}}
\newcommand{\bi}{{\vc{i}}}


\newcommand{\be}{\mbox{$\mathbf{e}$}}
\newcommand{\bx}{\mbox{$\mathbf{x}$}}
\newcommand{\bxi}{\mbox{$\mathbf{x}_i$}}
\newcommand{\byi}{\mbox{$\mathbf{y}_i$}}
\newcommand{\bzi}{\mbox{$\mathbf{z}_i$}}
\newcommand{\by}{\mbox{$\bf y$}}
\newcommand{\bz}{\mbox{$\bf z$}}
\newcommand{\bd}{\mbox{$\bf d$}}
\newcommand{\bxs}{\mbox{$\bf\scriptstyle x$}}
\newcommand{\bzs}{\mbox{$\bf\scriptstyle z$}}
\newcommand{\bys}{\mbox{$\bf\scriptstyle y$}}
\newcommand{\bzhat}{\mbox{$\hat{\bf z}$}}
\newcommand{\bp}{\mbox{$\bf p$}}
\newcommand{\bq}{\mbox{$\bf q$}}
\newcommand{\bs}{\mbox{$\bf s$}}
\newcommand{\bn}{\mbox{$\bf n$}}
\newcommand{\bh}{\mbox{$\bf h$}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\bm}{\mbox{$\bf m$}}
\newcommand{\bu}{\mbox{$\bf u$}}
\newcommand{\bv}{\mbox{$\bf v$}}
\newcommand{\bc}{\mbox{$\bf c$}}

\newcommand{\bA}{\mbox{$\bf A$}}
\newcommand{\bB}{\mbox{$\bf B$}}
\newcommand{\bC}{\mbox{$\bf C$}}
\newcommand{\bD}{\mbox{$\bf D$}}
\newcommand{\bE}{\mbox{$\bf E$}}
\newcommand{\bF}{\mbox{$\bf F$}}
\newcommand{\bG}{\mbox{$\bf G$}}
\newcommand{\bH}{\mbox{$\bf H$}}
\newcommand{\bI}{\mbox{$\bf I$}}
\newcommand{\bJ}{\mbox{$\bf J$}}
\newcommand{\bM}{\mbox{$\bf M$}}
\newcommand{\bL}{\mbox{$\bf L$}}
\newcommand{\bN}{\mbox{$\bf N$}}
\newcommand{\bP}{\mbox{$\bf P$}}
\newcommand{\bR}{\mbox{$\bf R$}}
\newcommand{\bS}{\mbox{$\bf S$}}
\newcommand{\bT}{\mbox{$\bf T$}}
\newcommand{\bU}{\mbox{$\bf U$}}
\newcommand{\bV}{\mbox{$\bf V$}}
\newcommand{\bW}{\mbox{$\bf W$}}
\newcommand{\bX}{\mbox{$\bf X$}}
\newcommand{\bY}{\mbox{$\bf Y$}}
\newcommand{\bZ}{\mbox{$\bf Z$}}
\newcommand{\bQ}{\mbox{$\bf Q$}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}


\newcommand{\vecy}{{\vc{y}}}
\newcommand{\tH}{\widetilde{{\bf H}}}

\newcommand{\px}{\mbox{$p(\x)$}}
\newcommand{\py}{\mbox{$p(\y)$}}

\newcommand{\exi}{\mbox{exp}\left(-\left\|\frac{\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\eyxz}{\mbox{exp}\left(-\left\|\frac{\y_j-\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\eyxo}{\mbox{exp}\left(-\left\|\frac{\y_{j+1}-\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\ey}{\mbox{exp}\left(\left\|\frac{\y_{j+1}}{\displaystyle{h}}\right\|^2\right)}

%%%%%%%%%%%%%%%%%%%%%% Kernel Density Stuff %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\myK}{K\left(\frac{\x-\x_{i}}{\displaystyle{h}}\right)}
\newcommand{\myKy}{K\left(\frac{\y^j-\x_{i}}{\displaystyle{h}}\right)}

\newcommand{\myG}{G\left(\frac{\x-\x_{i}}{\displaystyle{h}}\right)}

\newcommand{\myk}{k\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\myky}{k\left(\left\|\frac{\y^j-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\myki}{k\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}
\newcommand{\mykyi}{k\left(\left\|\frac{\y^j-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}

\newcommand{\myg}{g\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\mygy}{g\left(\left\|\frac{\y_j-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\mygi}{g\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}
\newcommand{\mygyi}{g\left(\left\|\frac{\y_j-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}

\newcommand{\mygd}{g\left(d^2(\mathbf{x},\mathbf{x}_i)/h^2\right)}

\newcommand{\MSE}{\mbox{MSE}}
\newcommand{\MISE}{\mbox{MISE}}



\newcommand{\lsup}[2]{\ensuremath{{}^{#1}\!{#2}}}
\newcommand{\hbo}[1]{\hat{{\bf #1}}}

%%%%%%%%  operators
\newcommand{\med}[1]{\mathop{\mbox{med}}\limits_{#1}}
\newcommand{\var}{\mbox{var}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\diag}{\mbox{\bf diag}}
\newcommand{\mytr}[1]{{\rm trace} [ #1 ]}
\newcommand{\mymax}[1]{\mathop{\mbox{max}}\limits_{#1}}
\newcommand{\mydet}[1]{{\rm det} [ #1 ]}
\newcommand{\vect}{\mbox{\bf vec}}

\newcommand{\myexps}{\mbox{exp}\left(-\frac{1}{2}\|\x\|^2\right)}
\newcommand{\maha}{{\rm D}\left[\x, \x_i, \bH\right]^2}
\newcommand{\mahai}{{\rm D}\left[\x, \x_i, \bH_i\right]^2}
\newcommand{\myexpm}{\mbox{exp}\left(-\frac{1}{2}\maha\right)}
\newcommand{\myexpmi}{\mbox{exp}\left(-\frac{1}{2}\mahai\right)}

\newcommand{\tr}{\mbox{tr\ }}



\newcommand{\myave}[1]{\mathop{\mbox{ave}}\limits_{#1}}

\newcommand{\ww}{{\vc{w}}}
\newcommand{\tbY}{\tilde\Y}

\newcommand{\bb}{\vc{b}}

\newcommand{\Jc}{\mathcal{J}}
\newcommand{\bzeta}{\vc{\zeta}}

